CTMCs with Imprecisely Timed Observations

Labeled continuous-time Markov chains (CTMCs) describe processes subject to random timing and partial observability. In applications such as runtime monitoring, we must incorporate past observations. The timing of these observations matters but may be uncertain. Thus, we consider a setting in which we are given a sequence of imprecisely timed labels called the evidence. The problem is to compute reachability probabilities, which we condition on this evidence. Our key contribution is a method that solves this problem by unfolding the CTMC states over all possible timings for the evidence. We formalize this unfolding as a Markov decision process (MDP) in which each timing for the evidence is reflected by a scheduler. This MDP has infinitely many states and actions in general, making a direct analysis infeasible. Thus, we abstract the continuous MDP into a finite interval MDP (iMDP) and develop an iterative refinement scheme to upper-bound conditional probabilities in the CTMC. We show the feasibility of our method on several numerical benchmarks and discuss key challenges to further enhance the performance.

==> Figures/Example/abstraction.tex <==
\tikzset{box around/.style={
    thick, draw=red, rounded corners,
    prefix after command= {\pgfextra{\tikzset{every label/.style={font=\scriptsize, yshift=-0.1cm, red, anchor=south west}}}}
}}

\begin{figure}[t]
\begin{subfigure}[b]{0.47\linewidth}
    \centering
    \iftikzcompile
    \begin{tikzpicture}[node distance=1.2cm]

    \def\xshift{0.3cm}
    \def\xshiftB{-0.5cm}
    \def\yshift{-0.3cm}
      % t0
      \node[state, small, initial,initial where=left, initial text=] (s0t0) {$0, 0$};
      \node[state, small, below of=s0t0, yshift=\yshift] (s1t0) {$1, 0$};
      \node[state, small, below of=s1t0, yshift=\yshift] (s2t0) {$2, 0$};
      % t1
      \node[state, small, right of=s0t0, xshift=\xshift] (s0t1a) {$0, \munderbar{t}_1$};
      \node[state, small, below of=s0t1a, yshift=\yshift] (s1t1a) {$1, \munderbar{t}_1$};
      \node[state, small, below of=s1t1a, yshift=\yshift] (s2t1a) {$2, \munderbar{t}_1$};
      \node[right of=s0t1a, xshift=\xshiftB] (s0t1b) {$\cdots$};
      \node[below of=s0t1b, yshift=\yshift] (s1t1b) {$\cdots$};
      \node[below of=s1t1b, yshift=\yshift] (s2t1b) {$\cdots$};
      \node[state, small, right of=s0t1b, xshift=\xshiftB] (s0t1c) {$0, \bar{t}_1$};
      \node[state, small, below of=s0t1c, yshift=\yshift] (s1t1c) {$1, \bar{t}_1$};
      \node[state, small, below of=s1t1c, yshift=\yshift] (s2t1c) {$2, \bar{t}_1$};
      %
      %t2
      \node[right of=s0t1c, xshift=\xshift] (s0t2) {$\cdots$};
      \node[below of=s0t2, yshift=\yshift] (s1t2) {$\cdots$};
      \node[below of=s1t2, yshift=\yshift] (s2t2) {$\cdots$};

      \node[box around, fit=(s0t1a) (s0t1c), label={above:${\langle s_0, \tilde\impT_1 \rangle}$}] (s0T1) {};
      \node[box around, fit=(s1t1a) (s1t1c), label={above:${\langle s_1, \tilde\impT_1 \rangle}$}] (s1T1) {};
      \node[box around, fit=(s2t1a) (s2t1c), label={above:${\langle s_2, \tilde\impT_1 \rangle}$}] (s2T1) {};
      
      \path[->] (s0t0) edge [] node [above] {} (s0T1)
                (s0t0) edge [] node [above] {} ($(s1T1.north west) + (0.1cm,0cm)$)
                (s0t0) edge [] node [above] {} ($(s2T1.north west) + (0.1cm,0cm)$)
                (s1t0) edge [] node [above] {} ($(s0T1.south west) + (0cm,0.1cm)$)
                (s1t0) edge [] node [above] {} (s1T1)
                (s1t0) edge [] node [above] {} ($(s2T1.north west) + (0cm,-0.1cm)$)
                (s2t0) edge [] node [above] {} ($(s0T1.south west) + (0.1cm,0cm)$)
                (s2t0) edge [] node [above] {} ($(s0T1.south west) + (0.1cm,0cm)$)
                (s2t0) edge [] node [above] {} (s2T1)
                %
                (s0T1) edge [red, thick, bend right=40] node [] {} (s0t0)
                ($(s1T1.east) + (0cm, 0.2cm)$) edge [] node [above] {} (s0t2)
                (s1T1.east) edge [] node [above] {} (s1t2)
                ($(s1T1.east) + (0cm, -0.2cm)$) edge [] node [above] {} (s2t2)
                ($(s2T1.east) + (0cm, 0.2cm)$) edge [] node [above] {} (s0t2)
                ($(s2T1.east) + (0cm, +0.1cm)$) edge [] node [above] {} (s1t2)
                (s2T1.east) edge [] node [above] {} (s2t2);               
    \end{tikzpicture}
    \fi
    \caption{Initial abstraction.}
\label{fig:abstraction1}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[b]{0.47\linewidth}
    \centering
    \iftikzcompile
    \begin{tikzpicture}[node distance=1.2cm]

    \def\xshift{0.3cm}
    \def\xshiftB{-0.5cm}
    \def\yshift{-0.3cm}
      % t0
      \node[state, small, initial,initial where=left, initial text=] (s0t0) {$0, 0$};
      \node[state, small, below of=s0t0, yshift=\yshift] (s1t0) {$1, 0$};
      \node[state, small, below of=s1t0, yshift=\yshift] (s2t0) {$2, 0$};
      % t1
      \node[state, small, right of=s0t0, xshift=\xshift] (s0t1a) {$0, \munderbar{t}_1$};
      \node[state, small, below of=s0t1a, yshift=\yshift] (s1t1a) {$1, \munderbar{t}_1$};
      \node[state, small, below of=s1t1a, yshift=\yshift] (s2t1a) {$2, \munderbar{t}_1$};
      \node[right of=s0t1a, xshift=\xshiftB] (s0t1b) {$\cdots$};
      \node[below of=s0t1b, yshift=\yshift] (s1t1b) {$\cdots$};
      \node[below of=s1t1b, yshift=\yshift] (s2t1b) {$\cdots$};
      \node[state, small, right of=s0t1b, xshift=\xshiftB] (s0t1c) {$0, \bar{t}_1$};
      \node[state, small, below of=s0t1c, yshift=\yshift] (s1t1c) {$1, \bar{t}_1$};
      \node[state, small, below of=s1t1c, yshift=\yshift] (s2t1c) {$2, \bar{t}_1$};
      %
      %t2
      \node[right of=s0t1c, xshift=\xshift] (s0t2) {$\cdots$};
      \node[below of=s0t2, yshift=\yshift] (s1t2) {$\cdots$};
      \node[below of=s1t2, yshift=\yshift] (s2t2) {$\cdots$};

      \coordinate (s0_left)  at ($(s0t1b) + (-0.2cm, 0cm)$);
      \coordinate (s0_right) at ($(s0t1b) + (0.2cm, 0cm)$);
      \coordinate (s1_left)  at ($(s1t1b) + (-0.2cm, 0cm)$);
      \coordinate (s1_right) at ($(s1t1b) + (0.2cm, 0cm)$);
      \coordinate (s2_left)  at ($(s2t1b) + (-0.2cm, 0cm)$);
      \coordinate (s2_right) at ($(s2t1b) + (0.2cm, 0cm)$);

      \node[box around, fit=(s0t1a) (s0_left), label={[anchor=south]above:${\langle s_0, \tilde\impT_1 \rangle}$}] (s0T1) {};
      \node[box around, fit=(s1t1a) (s1_left), label={[anchor=south]above:${\langle s_1, \tilde\impT_1 \rangle}$}] (s1T1) {};
      \node[box around, fit=(s2t1a) (s2_left), label={[anchor=south]above:${\langle s_2, \tilde\impT_1 \rangle}$}] (s2T1) {};

      \textbf{\node[box around, fit=(s0t1c) (s0_right), label={[anchor=south]above:${\langle s_0, \tilde\impT_2 \rangle}$}] (s0T2) {};
      \node[box around, fit=(s1t1c) (s1_right), label={[anchor=south]above:${\langle s_1, \tilde\impT_2 \rangle}$}] (s1T2) {};
      \node[box around, fit=(s2t1c) (s2_right), label={[anchor=south]above:${\langle s_2, \tilde\impT_2 \rangle}$}] (s2T2) {};}
      
      \path[->] (s0t0) edge [] node [above] {} (s0T1)
                (s0t0) edge [] node [above] {} ($(s1T1.north west) + (0.1cm,0cm)$)
                (s0t0) edge [] node [above] {} ($(s2T1.north west) + (0.1cm,0cm)$)
                (s1t0) edge [] node [above] {} ($(s0T1.south west) + (0cm,0.1cm)$)
                (s1t0) edge [] node [above] {} (s1T1)
                (s1t0) edge [] node [above] {} ($(s2T1.north west) + (0cm,-0.1cm)$)
                (s2t0) edge [] node [above] {} ($(s0T1.south west) + (0.1cm,0cm)$)
                (s2t0) edge [] node [above] {} ($(s0T1.south west) + (0.1cm,0cm)$)
                (s2t0) edge [] node [above] {} (s2T1)
                %
                (s0T1) edge [red, thick, bend right=40] node [] {} (s0t0)
                ($(s0T2.north west) + (0.1cm, 0.02cm)$) edge [red, thick, bend right=60] node [] {} (s0t0)
                ($(s1T2.east) + (0cm, 0.2cm)$) edge [] node [above] {} (s0t2)
                (s1T2.east) edge [] node [above] {} (s1t2)
                ($(s1T2.east) + (0cm, -0.2cm)$) edge [] node [above] {} (s2t2)
                ($(s2T2.east) + (0cm, 0.2cm)$) edge [] node [above] {} (s0t2)
                ($(s2T2.east) + (0cm, +0.1cm)$) edge [] node [above] {} (s1t2)
                (s2T2.east) edge [] node [above] {} (s2t2)
                ;               
    \end{tikzpicture}
    \fi
    \caption{Abstraction refinement step.}
\label{fig:abstraction1}
\end{subfigure}
%
\caption{Abstraction for one imprecise inspection $\langle[\underline{t}_1, \bar{t}_1], o_1\rangle \in \imphist$ into (a) a single copy of the CTMC encoding the full interval $\tilde\impT_1 = [\underline{t}_1, \bar{t}_1]$, and (b) the refinement into two copies, encoding $\tilde\impT_1 = [\underline{t}_1, \frac{\bar{t}_1+\underline{t}_1}{2}]$ and $\tilde\impT_2 = [\underline{t}_1, \frac{\bar{t}_1+\underline{t}_1}{2}]$, respectively. Note that not all transitions are shown in (b) to avoid cluttering.}
\label{fig:abstraction}
\end{figure}
